PINTO: Faithful Language Reasoning Using Prompt-Generated Rationales

Neural language models (LMs) have achieved impressive results on various language-based reasoning tasks by utilizing latent knowledge encoded in their own pretrained parameters. To make this reasoning process more explicit, recent works retrieve a rationalizing LM's internal knowledge by training or prompting it to generate free-text rationales, which can be used to guide task predictions made by either the same LM or a separate reasoning LM. However, rationalizing LMs require expensive rationale annotation and/or computation, without any assurance that their generated rationales improve LM task performance or faithfully reflect LM decision-making. In this paper, we propose PINTO, an LM pipeline that rationalizes via prompt-based learning, and learns to faithfully reason over rationales via counterfactual regularization. First, PINTO maps out a suitable reasoning process for the task input by prompting a frozen rationalizing LM to generate a free-text rationale. Second, PINTO's reasoning LM is fine-tuned to solve the task using the generated rationale as context, while regularized to output less confident predictions when the rationale is perturbed. Across four datasets, we show that PINTO significantly improves the generalization ability of the reasoning LM, yielding higher performance on both in-distribution and out-of-distribution test sets. Also, we find that PINTO's rationales are more faithful to its task predictions than those generated by competitive baselines.

==> tables/more_case_study.tex <==
\begin{table}[t]
\vspace{-0.6cm}
\centering
\caption{\small \textbf{Additional Case Study.} Generated rationales and model predictions from CSQA and StrategyQA.}
\label{tab:more_case_study}
%\vspace{-0.5cm}
\scalebox{0.85}{
\begin{tabular}{l|c|c}
\toprule
Questions and Choice-specific Rationales & Standard & PINTO \\
\midrule
\text{Q: What island country is ferret popular?}  &  \multirow{6}{*}{\text{great britain}~\color{red}\xmark} &\multirow{6}{*}{\text{great britain}~\color{green}\cmark}\\
\text{(a) own home: }\textit{\color{blue}Ferrets are popular in own home country.} &&\\
\text{(b) north carolina: }\textit{\color{blue} Ferrets are popular in north carolina.}&&\\
\text{(c) great britain: }\textit{\color{blue}Great Britain is the island country of ferrets.} &&\\
\text{(d) hutch: }\textit{\color{blue}Huts are popular in the island country of Great Britain.} &&\\
\text{(e) outdoors: }\textit{\color{blue}Ferrets are popular in outdoors.} &&\\
% ...&&\\
\midrule
\text{Q: Has every astronaut survived their space journey?} &\multirow{4}{*}{\text{yes}~\color{red}\xmark}&\multirow{4}{*}{\text{no}~\color{green}\cmark}\\
\text{yes: }\textit{\color{blue}Astronauts have died in space. For example, the Challenger astronauts} && \\
\textit{\color{blue}~~~~~~~died in the Challenger space shuttle explosion.} &&\\
\text{no: }\textit{\color{blue}~The first astronaut to die was Yuri Gagarin. Gagarin died in a plane crash.} && \\
\bottomrule
\end{tabular}
}
\vspace{-0.3cm}
\end{table}

==> tables/prompts_full.tex <==
\begin{table}[t]
\vspace{-0.9cm}
\centering
\small
\caption{\textbf{Rationalization Prompts.} Prompt for rationalization on CommonsenseQA. %Newlines between answer choices are omitted due to limited space. 
}
\label{tab:prompts}
\vspace{0.3cm}
\scalebox{0.95}{
\begin{tabularx}{\textwidth}{l}
\toprule
\textbf{Q}: What do people use to absorb extra ink from a fountain pen?\newline\textbf{Answer Choices}: (a) shirt pocket (b) calligrapher's hand (c) inkwell (d) desk drawer (e) blotter \newline \textbf{A}: The answer is blotter. \textit{\color{blue} Blotting paper absorbs liquids like ink well.} \\
\\
\textbf{Q}: What home entertainment equipment requires cable?\newline\textbf{Answer Choices}: (a) radio shack (b) substation (c) cabinet (d) television (e) desk \newline \textbf{A}: The answer is television. \textit{\color{blue} Cable can be fixed to a television. Television is a home entertainment equipment.} \\
\\
\textbf{Q}: The fox walked from the city into the forest, what was it looking for?\newline\textbf{Answer Choices}: (a) pretty flowers (b) hen house (c) natural habitat (d) storybook (e) dense forest \newline \textbf{A}: The answer is natural habitat. \textit{\color{blue} Forests are one of the main natural habitats of foxes. equipment.} \\
\bottomrule
\end{tabularx}
}
\vspace{-0.35cm}
\end{table}
